Long Range Tensor Correlations in Charge and Parity Projected Fermionic Molecular Dynamics

Within the framework of Fermionic Molecular Dynamics a method is developed to better account for long range tensor correlations in nuclei when working with a single Slater determinant. Single-particle states with mixed isospin and broken parity build up an intrinsic Slater determinant which is then charge and parity projected. By minimizing the energy of this many-body state with respect to the parameters of the single-particle states and projecting afterwards on angular momentum ground state energies are obtained that are systematically lower than corresponding Hartree-Fock results. The realistic Argonne V18 potential is used and short range correlations are treated with the Unitary Correlation Operator Method. Comparison with exact few-body calculations shows that in $^4$He about one fifth of the correlation energy due to long-range correlations are accounted for. These correlations which extend over the whole nucleus are visualized with the isospin and spin-isospin density of the intrinsic state. The divergence of the spin-isospin density, the source for pion fields, turns out to be of dipole nature.

==> ResultsFMD.tex <==
\subsection{FMD-interaction Besserer Titel!!!}





\begin{figure}[t]
\begin{center}
\rotatebox{0}{\includegraphics*[scale=0.5]{fig1.eps}}
\caption{(Color online) Convergence of the minimum of the charge and
  parity projected energy as a function of the number of points used
  in the charge projection operator, see Eq.~(\ref{charge_projector}):
  $^4$He case in upper panel and $^6$Li case in lower panel. One
  Gaussian per nucleon has been used.}
\label{figure1}
\end{center}
\end{figure}


We begin the discussion of our results by showing a test of
 the numerical accuracy for the minimization after charge  and parity projection procedure.
To investigate this,  we  look at the energy obtained from Eq.~(\ref{CPP}) in case we use an approximate charge projection $P_{\mathcal N}^{M_{T}}$, with ${\mathcal N} \le {A}$. This consists in taking a restricted number of rotations in isospin space for the charge projection of Eq.~(\ref{charge_projector}).
In Fig.~\ref{figure1}, we show  the convergence of the CPP energy
as a function of the number of points ${\mathcal N}$.
 We observe that, even if the
analytically exact projection is achieved when ${\mathcal N}= A$, numerically we reach stable
results already with 3 grid-points in the isospin projection.
This is  due to the fact that, via the VAP procedure, the component of the wave
function with different $T_z$  are simply dynamically suppressed during the minimization. The CPP state we obtain is ``optimized'' for the desired
third isospin component,  $M_T=0$ in the discussed case. In fact, if we project the obtained intrinsic state
$\left| Q \right\rangle$
 on $M_T=\pm 1$ and $M_T=\pm 2$ we will see that their norms are negligible.
Specifically, both for the above presented $A=4$ and $6$ cases, we find that
\beqa
\nonumber
\frac{\left\langle Q | \op{P}^{\pi}\op{P}^{M_T=\pm 1} | Q \right\rangle}
{\left\langle Q | \op{P}^{\pi}\op{P}^{M_T=0} | Q \right\rangle} < 10^{-1}\\
\frac{\left\langle Q | \op{P}^{\pi}\op{P}^{M_T=\pm 2} | Q \right\rangle}
{\left\langle Q | \op{P}^{\pi}\op{P}^{M_T=0} | Q \right\rangle}< 10^{-3} \,,
\eeqa
i.e. the higher $|T_z|$ component are at least two orders of magnitude smaller than the $T_z=0$ one.
The advantage, more important for increasing number of nucleons, is that one can perform an approximated projection obtaining an energy which has numerically the same accuracy as a full projection.


\begin{figure}[t]
\begin{center}
\rotatebox{0}{\includegraphics*[scale=0.35]{fig2.eps}}
\caption{(Color online) Comparison of CPP and HF binding energies for $T_z=0$ nuclei with different mass number $A$, obtained with one Gaussian packets per nucleon, using as NN interaction the potential in Eq.~(\ref{potential}).}
\label{figure2}
\end{center}
\end{figure}

It is now interesting to study the evolution of the charge and parity projected energy for different nuclei, once the projection on  the third component of isospin has converged.
In Fig.~\ref{figure2}, we show the CPP energies for $T_z=0$ nuclei,
ranging from mass number $4\le A \le 10$, and we compare them with the
values obtained by minimizing just the intrinsic energy, as intended
in Eq.~(\ref{HF}).
% using the single particle parameterization as in
% Eq.~(\ref{paramFMD}).
 The latter energies are hereafter denominated as Hartree-Fock calculations (HF), even if they are obtained with the FMD wave function using one Gaussian per nucleon.
One observes that the CPP energies are systematically lower than HF ones, as one would  naturally expect due to the fact that the wave function has additional degrees of freedom in isospin-space.
An other natural reason why the charge and parity projected  energies lie lower than the HF is that in the CPP procedure we actually minimize the energy of  a linear combination of states which are  rotations in isospin space  of the same SD. In other words, we are diagonalizing the Hamiltonian on a larger Hilbert space, thus the energy has to decrease for the variational principle.
The gain in binding energy  we obtain when going from the CPP to the HF strongly depends on the nuclear system under study:
 in case of  the stiff $\alpha$-particle the difference is just
  0.5 MeV, whereas $^6$Li and $^{10}$B  exhibit a softer behavior leading to
 an energy gain of 3-4 MeV.
Generally, the comparison with experiment improves, when using the CPP approach with respect to the HF. This is one first proof that
the description  of the long-range correlations is improved by mixing isospin
states, being  short-range correlations  already accounted for via
UCOM in the interaction (see Eq.~(\ref{potential})), which is the same
in both CPP and HF calculations. As expected, the ground
state energy for $^4$He is very close to the experiment, since the
interaction was fitted to this observable. On the other hand, for
other nuclei we still miss some MeV of binding with respect to the
experimental value (e.g. about $6$ MeV for $^{6}$Li). Clearly, we could improve the
description of these nuclei by performing a multiconfiguration
calculation with our CPP wave function. We leave this possible application for
future work.



